Ego-based Entropy Measures for Structural Representations

In complex networks, nodes that share similar structural characteristics often exhibit similar roles (e.g type of users in a social network or the hierarchical position of employees in a company). In order to leverage this relationship, a growing literature proposed latent representations that identify structurally equivalent nodes. However, most of the existing methods require high time and space complexity. In this paper, we propose VNEstruct, a simple approach for generating low-dimensional structural node embeddings, that is both time efficient and robust to perturbations of the graph structure. The proposed approach focuses on the local neighborhood of each node and employs the Von Neumann entropy, an information-theoretic tool, to extract features that capture the neighborhood's topology. Moreover, on graph classification tasks, we suggest the utilization of the generated structural embeddings for the transformation of an attributed graph structure into a set of augmented node attributes. Empirically, we observe that the proposed approach exhibits robustness on structural role identification tasks and state-of-the-art performance on graph classification tasks, while maintaining very high computational speed.

==> chapters/discussion.tex <==
\section{Discussion}
\subsection{Distributed computation}
Comment on the perspective of distributed computation of the local entropies that gives a more general picture of the graph
\subsection{Approximations of Von Neumann entropy}
Recently, research works have been published for more accurate approximations of the Von Neumann entropy. ...

==> chapters/preliminaries.tex <==
\section{Preliminaries}
For this work, we are going to focus on unattributed and undirected graphs, in order to emphasize in the expressiveness of the structural embeddings, that our algorithm provides. However, our method can be extended for the case where we have node attributes and directed edges. Firstly, we define the Laplacian eigenspectrum of a graph, the node's ego-network and then the notions of the Von Neumann entropy on graphs.

\subsection{Laplacian Eigenspectrum}

Let $G = (V, E)$ be a graph where $V$ is the set of nodes and $E$ is the set of edges. Let, also, $A \in \{0,1\}^{N\times N}$ be the adjacency matrix, where $N = |V|$ is the node set size. Using the adjacency matrix, we can define the Laplacian matrix $L = D - A$, where D is the degree matrix and its symmetric normalized version $~{L} = D^{-\frac{1}{2}}LD^{-\frac{1}{2}}$. The Laplacian eigenspectrum of the graph is provided by the eigendecomposition of the Laplacian: $L = U^T \Lambda U$, where U consists of the eigenvectors and $\Lambda = D(\lambda _1, \lambda _2, .., \lambda _n)$. Both versions of laplacians are symmetric and real valued, so their eigenvalues are all non-negative and we assume an ordering: $ 0 = \lambda _1 \leq \lambda_2 ... \leq \lambda _n $. Using the eigenspectrum of a graph is very often in the graph learning literature, as it exposes higher-level information regarding the structure of the graph.

% \subsection{Ego-networks of graph nodes}
% The majority of the literature usually employs the Laplacian eigenspectrum of the full graph, in order to exploit its structural characteristics. \citep{donat, DBLP:journals/corr/KipfW16, spectral_bruna}. In this work, we are focusing on computing local spectral characteristics, using the ego-network of the nodes inside a graph. That means, that for a specific given radius $r$, we focus on the induced subgraph centered by node $u$ $G_u'=(V',E')$ of the graph , where $V' = \{v \in V | d(u,v) \leq r\}$. In the laplacian field, that means, that we extract for every node $u$ the \textit{submatrix} $L_u'$ out of the total normalized Laplacian matrix $\~{L}$. For the rest of this work, we are going to refer to the normalized $\~{L}$ as $L$. 

\subsection{Von Neumann Entropy on graphs}
The term of Von Neumann entropy was firstly introduced in the field of quantum mechanics. A quantum system in a mixed state can be described by its \textit{density} matrix $\rho$.  Given that, the Von Neumann entropy of the quantum system is defined as: \begin{equation}
    \label{eq::1}
    H(\rho) = -tr(ln\rho)
\end{equation} and is a measure of the maximum amount of information that we can extract from a mixture of pure states. As soon as $\rho$ is a positive and semidefinite matrix, its eigenvalues follow:  $0 \leq \lambda_1 \leq \lambda_2, .. \leq \lambda_n$. Now, from the equation \ref{eq::1}, one can express the Von Neumann entropy as the Shannon Entropy of the spectrum of the density matrix:
\begin{equation}
\label{eq::2}
        H(\rho) = -\sum_{i=1}^n \lambda _i*ln\lambda _i
\end{equation}

%*** Des an symfwneis me th parakatv frash opws thn egrapsa 
Intuitively we can consider that the states of a quantum system are represented by the nodes of the graph density matrix.  Given a graph $G=(V,E)$ with its Laplacian $L$, its density matrix is defined as: $\rho (L) = \frac{L}{tr(L)} = \frac{L}{2*|E|}$. \citep{Braunstein2006}. Thus equation \ref{eq::2} can be used to compute the Von Neumann entropy for a graph.\\
% Intuitively we can consider Defining the sense of a density matrix in the context of graphs, we can have a correspondence between the states of a quantum system and the nodes of a graph.  Given a graph $G=(V,E)$ with its Laplacian $L$, its density matrix is defined as: $\rho (L) = \frac{L}{tr(L)} = \frac{L}{2*|E|}$. \citep{Braunstein2006}

% Now, the equation (2) expresses the Von Neumann entropy for a graph.\\
